CoinRobot: Generalized End-to-end Robotic Learning for Physical Intelligence

Physical intelligence holds immense promise for advancing embodied intelligence, enabling robots to acquire complex behaviors from demonstrations. However, achieving generalization and transfer across diverse robotic platforms and environments requires careful design of model architectures, training strategies, and data diversity. Meanwhile existing systems often struggle with scalability, adaptability to heterogeneous hardware, and objective evaluation in real-world settings. We present a generalized end-to-end robotic learning framework designed to bridge this gap. Our framework introduces a unified architecture that supports cross-platform adaptability, enabling seamless deployment across industrial-grade robots, collaborative arms, and novel embodiments without task-specific modifications. By integrating multi-task learning with streamlined network designs, it achieves more robust performance than conventional approaches, while maintaining compatibility with varying sensor configurations and action spaces. We validate our framework through extensive experiments on seven manipulation tasks. Notably, Diffusion-based models trained in our framework demonstrated superior performance and generalizability compared to the LeRobot framework, achieving performance improvements across diverse robotic platforms and environmental conditions.

==> texts/comparisonVC.tex <==
\section{Experiments and Results}
\label{sec:Experiments and Results}
%-------------------------------------------------
% insert table
% \begin{table*}[t]
% \centering
% \begin{tabular}{lcccccccccr}
% \hline
% \multicolumn{1}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}Task\\ Name\end{tabular}}} &
%   \textbf{\begin{tabular}[c]{@{}c@{}}Objects\\ Num\end{tabular}} &
%   \textbf{\begin{tabular}[c]{@{}c@{}}Receptacle\\ Num\end{tabular}} &
%   \textbf{Cases} &
%   \textbf{Color} &
%   \textbf{Size} &
%   \textbf{Shape} &
% \textbf{\begin{tabular}[c]{@{}c@{}}Logic\\ Step\end{tabular}} &
%   \textbf{\begin{tabular}[c]{@{}c@{}}Avg\\ Length\end{tabular}} &
%   \textbf{\begin{tabular}[c]{@{}c@{}}Demo\\ Num\end{tabular}} &
%   \multicolumn{1}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}Success\\ Rate\end{tabular}}} \\ \hline
% PickPlace        & 1 & 1 & 10 & No  & No  & No  & 1 & 16.35s & 280 & 92\%   \\
% BlockPick        & 2 & 2 & 10 & Yes & No  & No  & 2 & 24.02s & 330 & 74\%   \\
% Basketball       & 1 & 1 & 2  & No  & No  & No  & 1 & 22.07s & 100 & 92\%   \\
% RingToss         & 2 & 1 & 10   & Yes  & No  & No  & 2  & 40.28s & 100 & 72\%       \\
% CupStack         & 2 & 1 & 10 & Yes & No  & No  & 2 & 28.49s & 200 & 80\%   \\
% ShapeDistinguish & 1 & 1 & 10 & Yes & No  & Yes & 2 & 12.73s & 120 & 42\%   \\
% WhichCube        & 3 & 3 & 10 & No  & Yes & No  & 3 & 29.69s       & 80    & 35\%       \\
% PickSmall        & 1 & 1 & 6  & No  & Yes & No  & 2 & 11.93s & 60  & 66.7\%   \\
% PickBig          & 1 & 1 & 6  & No  & Yes & No  & 2 & 11.88s & 120 & 76.6\% \\
% PickBigV2        & 1 & 1 & 12 & No  & Yes & No  & 2 & 12.00s & 240 & 78.3\% \\ \hline
% \end{tabular}
% \caption{\textbf{Overview of task characteristics}: \textbf{Objects Num} refers to the number of objects the robot interacts with; \textbf{Receptacle Num} indicates the number of possible changes to the receptacle; \textbf{Cases} specifies the number of initial conditions; \textbf{Color}, \textbf{Size}, and \textbf{Shape} indicate whether the task involves classifying these features; \textbf{Logic Step} represents the number of logical deductions required; \textbf{Avg Length} is the average duration of each demonstration video; \textbf{Demo Num} denotes the total number of demonstrations for each task.}
% \label{tab:task_performance}
% \end{table*}
%-------------------------------------------------------


\subsection{Task Analysis}
Following the standardized checkpoint selection method discussed in Section \ref{sec:Checkpoint Selection}, we present our analysis of the relationship between task success rates and task-specific characteristics. To minimize the impact of model architecture and training strategy, we utilized a consistent architecture and selected the optimal checkpoint based solely on performance, regardless of training duration.

Table \ref{tab:task_performance} summarizes the manual feature extractions for each task, along with corresponding dataset sizes. While it is difficult to establish a direct linear relationship between task features and success rates, our findings suggest the following key perceptions:

\begin{enumerate}
    \item \textbf{Number of Demonstrations}: The number of demonstrations significantly influences the final success rate. This is evident in tasks such as 'PickSmall,' 'PickBig,' and 'PickBigV2,' which serve as controlled experiments where the dataset size is the primary variable. The success rate increases as the dataset size grows, but plateaus at a certain threshold.
    
    \item \textbf{Task Complexity}: Task complexity is directly correlated with the Voting Positive Rate (VPR). As expected, tasks that require more complex decision-making—such as those involving multiple sequential steps—tend to be more challenging. To quantify this, we introduce a manually defined marker, \textbf{Logic Step}, which represents the number of logical deductions a human would need to make to control the robot arm. This concept is inspired by the use of Chain-of-Thought prompting in Large Language Models \cite{c3,c4}..
    
    \item \textbf{Feature Distinguishability}: Based on practical experience, tasks that prominently feature color differentiation appear to benefit more from the ResNet-based perception encoder. This suggests that the current architecture is particularly effective for tasks where visual color features are critical.
\end{enumerate}

\subsection{Model Architecture Ablation Study}
%-------------------------------------------------
% insert table
% \begin{table*}[ht]
% \centering
% \begin{tabular}{lcccc}
% \toprule
% \textbf{Task Name}        & \textbf{ResNet18+UNet} & \textbf{ResNet18+Transformer} & \textbf{ResNet34+Transformer} & \textbf{FPN+Transformer} \\
% \midrule
% PickPlace        & 92\% & 92\%   & 80\%    & \textbf{95\%}    \\
% BlockPick        & 63\%   & 74\% & 56\% & 70\%  \\
% Basketball       & 92\% & \textbf{92\%}   & 80\%    & 86.7\%    \\
% CupStack         & 26\%     & 57.5\% & 70\%  & \textbf{80\%}  \\
% RingToss         & 26\%     & 60\% & 70\%    & \textbf{72\%}    \\
% ShapeDistinguish & 16.7\%     & 33\% & 20\%    & \textbf{42\%}    \\
% WhichCube        & 8.3\%     & 33\%    & \textbf{35\%}    & \textbf{35\%}    \\
% PickSmall        & 16.7\% & 20\% & \textbf{66.7\%} & 60\%  \\
% PickBig          & 26.7\%    & 50\% & 26.7\% & \textbf{76.6\%} \\
% PickBigV2        & 45\%   & 55.7\% & 50\% & \textbf{78.3\%} \\
% \bottomrule
% \end{tabular}
% \caption{The optimal Voting Positive Rate (VPR) for four different model architectures across 10 tasks. Each model checkpoint was selected based on exhaustive evaluation.}
% \label{tab:ablation_study}
% \end{table*}
%-------------------------------------------------

%------

% Please add the following required packages to your document preamble:
% \usepackage{multirow}

\begin{table*}[htbp]
\centering
\begin{tabular}{lcccccccccrrrrr}
\hline
\multicolumn{1}{c}{\multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Task\\ Name\end{tabular}}}} &
  \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Object\\ Num\end{tabular}}} &
  \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Recept\\ Num\end{tabular}}} &
  \multirow{2}{*}{\textbf{Cases}} &
  \multirow{2}{*}{\textbf{Color}} &
  \multirow{2}{*}{\textbf{Size}} &
  \multirow{2}{*}{\textbf{Shape}} &
  \multirow{2}{*}{\textbf{Logic}} &
  \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Avg\\ Length\end{tabular}}} &
  \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Demo\\ Num\end{tabular}}} &
  \multicolumn{4}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}Success Rate\end{tabular}}} \\ \cline{11-14} 
\multicolumn{1}{c}{} &
   &
   &
   &
   &
   &
   &
   &
   &
   &
  \scriptsize\textbf{\begin{tabular}[c]{@{}l@{}}DP-CNN\end{tabular}} &
  \scriptsize\textbf{\begin{tabular}[c]{@{}l@{}}DP-TF\end{tabular}} &
  \scriptsize\textbf{\begin{tabular}[c]{@{}l@{}}ChengLingV1\end{tabular}} &
  \scriptsize\textbf{\begin{tabular}[c]{@{}l@{}}ChengLingV2\end{tabular}} \\ \hline

BlockPick &
  2 &
  2 &
  10 &
  Yes &
  No &
  No &
  2 &
  24.02s &
  330 &
  63\% &
  \textbf{74\%} &
  56\% &
  70\% \\

RingToss &
  2 &
  1 &
  10 &
  Yes &
  No &
  No &
  2 &
  40.28s &
  100 &
  26\% &
  60\% &
  70\% &
  \textbf{72\%} \\
CupStack &
  2 &
  1 &
  10 &
  Yes &
  No &
  No &
  2 &
  28.49s &
  200 &
  26\% &
  57.5\% &
  70\% &
  \textbf{80\%} \\
ShapeDistinguish &
  1 &
  1 &
  10 &
  Yes &
  No &
  Yes &
  2 &
  12.73s &
  120 &
  16.7\% &
  33\% &
  20\% &
  \textbf{42\%} \\
WhichCube &
  3 &
  3 &
  10 &
  No &
  Yes &
  No &
  3 &
  29.69s &
  80 &
  8.3\% &
  33\% &
  \textbf{35\%} &
  \textbf{35\%} \\
PickSmall &
  1 &
  1 &
  6 &
  No &
  Yes &
  No &
  2 &
  11.93s &
  60 &
  16.7\% &
  20\% &
  \textbf{66.7\%} &
  60\% \\
PickBig &
  1 &
  1 &
  6 &
  No &
  Yes &
  No &
  2 &
  11.88s &
  120 &
  26.7\% &
  50\% &
  26.7\% &
  \textbf{76.6\%} \\
PickBigV2 &
  1 &
  1 &
  12 &
  No &
  Yes &
  No &
  2 &
  12.00s &
  240 &
  45\% &
  55.7\% &
  50\% &
  \textbf{78.3\%} \\ \cline{1-14}
\end{tabular}
\caption{\textbf{Overview of task characteristics}: \textbf{Object Num} refers to the number of objects the robot interacts with; \textbf{Recept Num} indicates the number of possible changes to the receptacle; \textbf{Cases} specifies the number of initial conditions; \textbf{Color}, \textbf{Size}, and \textbf{Shape} indicate whether the task involves classifying these features; \textbf{Logic Step} represents the number of logical deductions required; \textbf{Avg Length} is the average duration of each demonstration video; \textbf{Demo Num} denotes the total number of demonstrations for each task. \textbf{Model structure abbreviations:} \textbf{DP-CNN} refers to DP with ResNet18 and CNN architecture, \textbf{DP-TF(Transformer)} refers to DP with ResNet18 and Transformer-based architecture, \textbf{ChengLing-V1} refers to proprietary architecture v1, and \textbf{ChengLing-V2} refers to proprietary architecture v2. Each model checkpoint was selected based on exhaustive evaluation mentioned on Section \ref{sec:Checkpoint Selection}.}
\label{tab:task_performance}
\end{table*}
%------
As aforementioned \ref{sec:Policy Control System}, we decoupled the whole controlling system into perception module and action prediction module, and each of them can be instanced by certain network architectures. Hence, we conducted an ablation study to evaluate the performance of various model architectures by modifying both of them. As shown in Table \ref{tab:task_performance}, the study compares the performance of ResNet18 with a CNN based module, and ResNet18, ResNet34, and FPN-based ResNet34 with transformer-based across different tasks.

% We conducted an ablation study to evaluate the performance of various model architectures by modifying both the perception encoder and the noise prediction network. As shown in Table \ref{tab:ablation_study}, the study compares the performance of ResNet18 with a UNet-based noise prediction network, and ResNet18, ResNet34, and FPN-based ResNet34 with transformer-based noise prediction networks across different tasks.

For simpler tasks such as PickPlace and Basketball, the ResNet18+UNet architecture achieved relatively good VPR, with a notable 92\% rate. This indicates that CNN-based noise prediction networks are effective when the task complexity is relatively low, likely due to their ability to capture local spatial patterns efficiently.

However, transformer-based architectures perform generally better compared to CNN-based. When task complexity increased, the outnum becomes larger. Transformers particularly excelled in the most complex tasks, such as PickSmall, where ResNet34+Transformer outperformed all other architectures with a 66.7\% success rate. This confirms that transformers are well-suited for handling tasks requiring more sophisticated temporal and spatial reasoning, as their self-attention mechanism allows them to capture long-range dependencies more effectively than CNNs.

Among Transformer group, FPN+Transformer is considered as the optimal choice, as it generally perform better. For instance, in the CupStack task, the FPN+Transformer architecture outperformed others, achieving an 80\% success rate, compared to 70\% for ResNet34+Transformer and 57.5\% for ResNet18+Transformer. Similarly, in the PickBig task, FPN+Transformer achieved 76.6\%, significantly outperforming the ResNet18+Transformer (50\%) and ResNet34+Transformer (26.7\%). When simply enlarge the perception model (e.g., from ResNet18 to ResNet34), the improvement of performance is not significant, ResNet34 even perfor worse on some simple tasks (e.g., 'PickPlace', 'BlockPick' and 'Basketball').

The ablation study underscores that while CNN-based architectures may perform well in simpler environments, transformer-based architectures offer a clear advantage in complex, dynamic tasks. These results suggest that, for tasks requiring intricate action sequences and environmental interactions, transformer-based models should be prioritized for their robustness and performance.

% However, as task complexity increased, the performance of transformer-based architectures became more prominent. For instance, in the CupStack task, the FPN+Transformer architecture outperformed others, achieving an 80\% success rate, compared to 70\% for ResNet34+Transformer and 57.5\% for ResNet18+Transformer. Similarly, in the PickBig task, FPN+Transformer achieved 76.6\%, significantly outperforming the ResNet18+Transformer (50\%) and ResNet34+Transformer (26.7\%).

% Transformers particularly excelled in the most complex tasks, such as PickSmall, where ResNet34+Transformer outperformed all other architectures with a 66.7\% success rate. This confirms that transformers are well-suited for handling tasks requiring more sophisticated temporal and spatial reasoning, as their self-attention mechanism allows them to capture long-range dependencies more effectively than CNNs.

\subsection{Dataset Scaling Matters More Than Training Scaling}
\label{sec:Dataset Scaling Matters}
We explicitly explored the effects of scaling both the dataset size and the model architecture by introducing additional demonstrations and increasing the model's hidden dimensions (i.e., adding more learnable parameters) alongside extended training epochs. Interestingly, our results indicate that simply increasing the number of model parameters and training time does not lead to improved performance. In fact, this approach often results in a significant drop in performance, rendering the model's success rate unacceptably low.

Conversely, increasing the number of demonstrations consistently improves model performance, as evidenced by the results from the ‘PickSmall’, ‘PickBig’, and ‘PickBigV2’ tasks. These three tasks were deliberately designed to be similar, with the primary difference being the number of demonstrations. The results are compelling: by increasing the number of demonstrations from 60 to 120, the VPR improves by 9.9\%. However, this improvement tends to plateau; when increasing the demonstrations from 120 to 240, the VPR only improves by 1.7\%. In addition to expanding the dataset, we also experimented with using a larger transformer model, but the results were far from expected. Although we aimed to replicate the scaling laws’ success observed in other domains by simultaneously increasing both dataset size and model complexity, our findings indicate that this strategy requires further exploration to be successfully applied.

\subsection{Data Quality}
\label{sec:Data quality}
During our experiments, we identified a recurring data quality issue, which we present here. When two data collectors independently gathered data for the same tasks, we observed significant variations in model performance, even when the demonstration lengths and training epochs were kept constant. These findings were consistent across most of the tasks we designed, particularly for tasks with longer demonstrations. While it is possible that this performance fluctuation could be attributed to the checkpoint selection problem mentioned earlier, we are inclined to believe it is more closely related to the proficiency level of the data collectors \cite{c1, c2}. However, the definition of “proficiency” remains unclear to us. Therefore, we are simply reporting our perceptions here and leave this question open for further investigation by our peers.

\subsection{Model Generalization}
\label{sec:Model Generalization}
\subsubsection*{Multi-task Generalization}
Similar to the early stages of deep learning, prior work in imitation learning has predominantly focused on training models for single, specific tasks. In contrast, we have developed a multi-task learning approach by combining two datasets and training on a pre-existing checkpoint that was already fine-tuned on one of the tasks. The efficacy of this approach was demonstrated by fine-tuning the ‘BlockPick’ task using a model checkpoint previously trained on the ‘Basketball’ task for 650 epochs. Remarkably, the ‘BlockPick’ task was successfully completed after only 50 additional epochs of fine-tuning, underscoring the efficiency and effectiveness of our multi-task learning strategy.
% The multi-task model offers several advantages:
% \begin{enumerate}
%     \item \textbf{Mitigation of Overfitting}: The multi-task model significantly reduces the risk of overfitting to a single task.
%     \item \textbf{Enhanced Generalization}: The model benefits from exposure to a diverse training dataset, encompassing variations in time of day, lighting conditions, and environmental objects, which contributes to improved generalization across different contexts.
% \end{enumerate}

\subsubsection*{Environmental Scene Generalization}
In standard imitation learning setups, demonstration data is typically collected with fixed camera positions, commonly involving one global view and another camera mounted on the end effector. This setup requires identical camera positions and view angles during inference to replicate the training conditions. Consequently, models trained under these constraints often exhibit limited adaptability and generalization to even minor variations in camera placement in real-world scenarios.
By incorporating merely two distinct camera views, with one camera fixed and the other placed at two different positions (each providing 40 demonstrations), we fine-tuned the model for an additional 100 epochs. Notably, in the 'BlockPick' task, this fine-tuning with multi-angle camera data enabled the model to maintain high performance despite variations in camera positioning, including zero-shot \cite{c53} positions and angles that were entirely unseen during the training phase. This result indicates that the model achieved robust generalization across a range of environmental visual conditions.

% \subsection{Model Training Insights}
% \label{sec:Model Training Insights}
% \subsubsection{Fine-tuning Pre-trained Models}
% Fine-tuning models based on pre-trained tasks resulted in superior performance and faster convergence compared to training a multi-task model from scratch.
% \subsubsection{Data Importance versus Epoch Count}
% The multi-task model, fine-tuned with just 50 additional epochs on a pre-trained model (initially trained for 650 epochs) using 80 additional data points from the second task, highlighted that the quality and relevance of the data are more critical to achieving high performance than the sheer number of training epochs.
% \subsubsection{Forgetting Effect}
% The phenomenon of catastrophic forgetting was observed when the multi-task model was fine-tuned exclusively on the second task's data, resulting in failure to perform the original task. In contrast, fine-tuning with both datasets allowed the model to successfully perform both tasks, indicating the necessity of integrated training to preserve task performance.
